Search and study of young infrared stellar clusters

The main aim of this paper is to study both the Interstellar Medium (ISM) and the young stellar population in the three star-forming regions, namely IRAS 05137+3919, 05168+3634, and 19110+1045. The study of the ISM includes determination of the hydrogen column density (N(H_2)) and dust temperature (T_d) in the regions using Modified blackbody fitting. The main parameters of identified and classified young stellar objects (YSOs) belonging to the regions were determined comparing with the radiation transfer models. We also constructed a colour-magnitude diagram to compare the parameters of the YSOs with the results of the radiative transfer models. The three stellar populations appear to have formed under different scenarios. In the cases of IRAS 05137+3919 and IRAS 05168+3634, the age spread is considerably wider, suggesting that the stellar population likely emerged from independent condensations. In contrast, the third region comprises a pair of ultra-compact HII regions (UCHIIs), G45.12+0.13 and G45.07+0.13, with a notably smaller age spread. This hints at the possibility that these clusters originated from a single triggering event.

==> proof.tex <==
\begin{document}

\begin{frontmatter}

\dochead{Research}% Updated by JobSheet2LaTeX.exe, 29.03.2024 09:35
%\subdochead{}
%\title{}
\title{Search and study of young infrared stellar clusters}
%\runtitle{}
\runtitle{Search and study of young infrared stellar clusters}

%%% initials in inits and fnm (if any) without spaces
%
%\begin{aug}
% [id=?,addressref=?,corref=?,presentaddressref=?]{\inits{}\fnm{}\particle{}~\snm{}\suffix{}\ead[label=?]{}\orcid{}}
%
%\author[id=au1,addressref=aff1,corref=aff1]{\inits{}\fnm{}~\snm{}\ead[label=e1]{}}
%\author[id=,addressref=]{\inits{}\fnm{}~\snm{}}
%\author[id=,addressref=]{\inits{}\fnm{}~\snm{}}
%
%\address[id=aff1]{%
%\orgdiv{},
%\orgname{},
%\street{},
%\city{},
%%\state{}
%\postcode{},
%\cny{}}
%
%\address[id=]{%
%%\orgdiv{},
%%\orgname{},
%%\street{},
%\city{},
%%\state{}
%%\postcode{},
%\cny{}}
%
%%\runauthor{} %auto
%\end{aug}
\begin{aug}
\author[id=au1,addressref=aff1,corref=aff1]{\inits{N.}\fnm{Naira}~\snm{Azatyan}\ead[label=e1]{nayazatyan@bao.sci.am}}
\address[id=aff1]{\orgname{Byurakan Astrophysical Observatory},
    \street{0213 Aragatsotn Prov.},
    \city{Byurakan vil.},
    \cny{Armenia}}
\end{aug}

\begin{history}
\received{\sday{13} \smonth{10} \syear{2023}}% Updated by JobSheet2LaTeX.exe, 29.03.2024 09:35
%\revised{\sday{} \smonth{} \syear{}}
\accepted{\sday{27} \smonth{3} \syear{2024}}% Updated by JobSheet2LaTeX.exe, 29.03.2024 09:35
\registered{\sday{27} \smonth{3} \syear{2024}}% Updated by JobSheet2LaTeX.exe, 29.03.2024 09:35
%\pubonline{\sday{} \smonth{} \syear{}}
\end{history}

%\begin{artnotes}
%\presentedat{}
%\presented{}
%\dedication{}
%\communicated{}
%\misc{}
%\crosslinking
%\corrigendum{}
%\ESMHint{The online version contains supplementary material available at \theshortdoi.}
%\motto{}
%\end{artnotes}

\printaddresses{}

%\begin{abstract}
%%\parttitle{} - NOT allowed, delete "parttitle" title + AQF
%\end{abstract}
\begin{abstract}
The main aim of this paper is to study both the Interstellar Medium (ISM) and the young stellar population in the three star-forming regions, namely IRAS 05137$+$3919, 05168$+$3634, and 19110$+$1045. The study of the ISM includes determination of the hydrogen column density (N(H$_{2}$)) and dust temperature (T$_{d}$) in the regions using modified blackbody fitting. The main parameters of the identified and classified young stellar objects (YSOs) belonging to the regions were determined by comparing with the radiation-transfer models. We also constructed a color--magnitude diagram to compare the parameters of the YSOs with the results of the radiative-transfer models. The three stellar populations appear to have formed under different scenarios. In the cases of IRAS 05137$+$3919 and IRAS 05168$+$3634, the age spread is considerably wider, suggesting that the stellar population likely emerged from independent condensations. In contrast, the third region comprises a pair of ultracompact HII regions (UCHIIs), G45.12$+$0.13 and G45.07$+$0.13, with a notably smaller age spread. This hints at the possibility that these clusters originated from a single triggering event.
\end{abstract}

%% all u.c.
%\begin{keyword}
%\kwd{}
%\end{keyword}
\begin{keyword}
\kwd{Stars: premain sequence}
\kwd{Infrared: stars}
\kwd{Radiative transfer}
\kwd{Interstellar medium (ISM)}
\end{keyword}

%\begin{keyword}[class=MSCnoyear]
%\kwd[Primary ]{}
%\kwd[\sep Secondary ]{}
%\end{keyword}

%\begin{abbrgroup}[width={}]
%\item[]
%\end{abbrgroup}

\end{frontmatter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Main text entry area:

%s1 #&#
\section{Introduction}
\label{sec1}

The process of star formation remains ongoing throughout various stages
of evolution of our galaxy and other galaxies, even in the present era
\citep{Ambartsumian47}. It stands as one of the most pivotal processes that
yield observable outcomes within galaxies. Giant molecular clouds are the
birthplaces of stellar populations \citep{Soderblom10}. Stellar clusters
that remain embedded within their original molecular clouds hold a special
significance. They provide insights into distinguishing the characteristics
of stellar clusters related to their birth conditions from those derived
from subsequent evolution \citep{lada03}. Therefore, there exists a genetic
connection between young stellar objects (YSOs) and the surrounding Interstellar
Medium (ISM). It necessitates an integrated approach to study star-forming
regions that implies determination of the main properties of already formed
young stellar clusters and the surrounding environment. Moreover, the integrated
approach to the study of embedded stellar clusters can provide information
about the initial star-formation scenarios. When star formation within
clusters is triggered, one would expect a limited age spread among the
stars within the cluster. Conversely, in protocluster condensations that
initiate star formation independently, individual clumps are likely to
exhibit a broader age distribution \citep[e.g., ][]{Preibisch12}.

This paper presents findings of a detailed investigation of young stellar
clusters in the three star-forming regions: IRAS 05137$+$3919, 05168$+$3634,
and 19110$+$1045 with a substantial size and multicomponent structures. All
three regions are active knots for star formation. Figure~\ref{fig:regions} shows color-composite images of the three star-forming
regions with combinations of different wavelength-range images. For each
of these regions, an exhaustive analysis was undertaken, covering the following
topics: 1) determining ISM parameters, specifically the distribution of
hydrogen column density (N(H$_{2}$)) and dust temperature (T$_{d}$); 2)
the search for young stellar clusters; 3) identifying cluster members by
examining their infrared characteristics; and 4) determining the age and
age spread among the members within these clusters. This paper is essentially
a generalization of the results presented in a series of works devoted
to the above-mentioned topics
\citep{Nikoghosyan14,azatyan16,Azatyan18,Azatyan19,Nikoghosyan20,Azatyan20,Nikoghosyan21,Azatyan22},
which were the basis for my PhD thesis.

We have organized the paper as follows. Section~\ref{2} describes the used
data and methods; in Sect.~\ref{3}, we analyze the stellar population
and ISM properties in the regions. Finally, the study results are summarized
in Sect.~\ref{4}.

%f1 #&#
\begin{figure*}
\includegraphics{4298f01}
\caption{(\textit{Left}) A color-composite image of the IRAS 05137$+$3919
star-forming region, combining data of UKIDSS J (in blue), H (in green),
and K (in red). The position of the IRAS source is marked by a black cross.
(\textit{Right}) A color-composite image of the G45.12$+$0.13 and G45.07$+$0.13
UCHII regions, combining data of Spitzer 5.0~\textmu m (in blue), Herschel
70~\textmu m (in green), and Herschel 160~\textmu m (in red). The positions
of the IRAS sources are marked by black crosses and they are in the following
order from top to bottom: IRAS 19111$+$1048 and 19110$+$1045. (\textit{Bottom})
A color-composite image of the IRAS 05168$+$3634 star-forming region, combining
data of WISE 12~\textmu m (in blue), Herschel 160~\textmu m (in green), and
Herschel 500~\textmu m (in red). The positions of the IRAS sources are marked
by black crosses and they are in the following order from the left to the
right: IRAS 05184$+$3635, 05177$+$3636, 05168$+$3634, 05162$+$3639, and 05156$+$3643.}
\label{fig:regions}
\end{figure*}
%%LEAP%%%\label{fig1}


%s2 #&#
\section{Used data and methods}
%%LEAP%%%\label{sec2}
\label{2}

The study encompasses two primary scientific aims: the examination of the
ISM and the analysis of YSOs. For this purpose, we used data covering a
wide range of near- to far-infrared (NIR, FIR) wavelengths.

For the determination of N(H$_{2}$) and T$_{d}$ in the three star-forming
regions, we used \textit{Herschel} FIR images, covering the optically thin
spectral range of 160--500~\textmu m obtained on the Photodetector Array
Camera and Spectrometer \citep[PACS,][]{poglitsch10} and the Spectral and
Photometric Imaging Receiver \citep[SPIRE,][]{griffin10}. These spectral
ranges are most productive for determining the parameters of the cold ISM
in molecular clouds. Dust emission in the FIR can be modeled as a modified
blackbody I$_{\nu}=k_{\nu}\mu _{H_{2}}m_{H}N(H_{2})B_{\nu}(T_{d})$, where
$k_{\nu}$ is the dust opacity, $\mu _{H_{2}} = 2.8$ represents the mean
weight per hydrogen molecule \citep{Kauffmann08}, $m_{H}$ is the mass of
hydrogen, $N(H_{2})$ is the hydrogen column density, and
$B_{\nu}(T_{d})$ is the Planck function at the dust temperature
$T_{d}$. The dust opacity in the FIR is usually parametrized as a power
law normalized to the value $k_{0}$ at a reference frequency
$\nu _{0}$, so k$_{\nu} = k_{0}(\nu /\nu _{0})^{\beta}\,cm^{-2}g^{-1}$.
Following \citet{hildebrand83}, \citet{Konyves15}, we adopted k$_{0} = 0.1$~cm$^{-2}g^{-1}$
at 300~\textmu m (gas-to-dust ratio of 100) and $\beta  = 2$.
\citet{roy2014} showed that this assumption is good within better than
50\% in the bulk of molecular clouds. Based on the discussion in previous
studies \citep[e.g.,][]{Battersby11}, we excluded the 70~\textmu m data
as the optically thin assumption may not hold. In addition, the emission
here would have a significant contribution from a warm dust component,
thus, modeling with a single-temperature blackbody would overestimate the
derived temperature. The three shortward intensity maps were degraded to
the spatial resolution of the 500~\textmu m band; the four maps were then
translated to a common coordinate system using 14\"  pixels at all wavelengths.
The SED fitting procedure for the cold ISM was executed pixel by pixel.
Following \citet{pezzuto2021}, we created a grid of models by varying only
the temperature, in the range 5 $\le $ T$_{d}(K)\le 50$, in steps
of 0.01~K and for each temperature $T_{j}$, the code computes the intensity
at FIR wavelengths for all bands. Since the intensity $I_{\nu}$ is linear
with $N(H_{2})$, we can compute the column density at each pixel using
a straightforward application of the least-squares technique. The uncertainty
of $I_{\nu}$ for SPIRE is 10\% and for PACS it is 20\%
\citep{Konyves15}. Figure~\ref{fig:SED} shows an example of blackbody fitting
for a low dust temperature (11~K) in IRAS 05137$+$3919 star-forming region.
The uncertainty between the observed and predicted fluxes is 0.024 for
this particular pixel.

%f2 #&#
\begin{figure}
\includegraphics{4298f02}
\caption{A blackbody fitting of a low dust temperature (11~K) in IRAS 05137$+$3919
star-forming region. The filled triangles represent the observed fluxes
in \textit{Herschel} four bands with their error bars, while filled circles
represent the fluxes predicted by the model in the same bands. The blue
line shows the fit of the predicted fluxes. The uncertainty between the
two samples is 0.024.}
\label{fig:SED}
\end{figure}
%%LEAP%%%\label{fig2}


For the second task, i.e., the analysis of YSOs, we used data spanning
the NIR, midinfrared (MIR), and FIR wavelengths. For this task, we used
the data of Galactic Plane Survey DR6 \citep[UKIDSS GPS,][]{lucas08}, Two
Micron Sky Survey \citep[2MASS,][]{Cutri03}, Galactic Legacy Infrared Midplane
Survey Extraordinaire (GLIMPSE) and GLIMPSE 360 \citep{churchwell09},
Multiband Infrared Photometer for \textit{Spitzer}
\citep[MIPSGAL,][]{Carey09}, Wide-field Infrared Survey Explorer
\citep[WISE,][]{wright10}, Midcourse Space Experiment
\citep[MSX, ][]{Price01}, \textit{Herschel} PACS, SPIRE, \textit{Herschel}
Infrared Galactic Plane Survey \citep[Hi-GAL,][]{molinari16}, and the Infrared
Astronomical Satellite \citep[IRAS,][]{Neugebauer84} Point Source Catalog
v2.1 (PSC) catalogs. The UKIDSS-DR6 catalog was selected as a primary.
Then, this catalog was crossmatched with other MIR and FIR catalogs, using
a matching radius of 3 $\sigma $, accounting for the combined error. Since
the presence of circumstellar discs and envelopes causes an infrared (IR)
excess of a YSO, YSO candidates were identified based on their position
in color--color (c--c) IR diagrams. The choice of colors relied on the
availability of data. We employed two c--c diagrams, specifically (J--H)
versus (H--K) and (J--K) versus [3.6]--[4.5], to identify YSOs within the
IRAS 05137$+$3919 star-forming region. Then, the selection of YSOs in the
IRAS 05168$+$3634 star-forming region was guided by the analysis of four
c--c diagrams, specifically (J--H) versus (H--K), K--[3.6] versus [3.6]--[4.5],
[3.4]--[4.6] versus [4.6]--[12], and [3.4]--[4.6] versus [4.6]--[22]. Finally,
the selection of YSOs in the IRAS 19110$+$1045 star-forming region involved
the utilization of six c--c diagrams, specifically (J--H) versus (H--K),
K--[3.6] versus [3.6]--[4.5], [3.6]--[4.5] versus [5.8]--[8.0], [3.6]--[5.8]
versus [8.0]--[24], [3.4]--[4.6] versus [4.6]--[12], and [3.4]--[4.6] versus
[4.6]--[22]. To validate the selected YSOs and extract their essential
characteristics, we constructed their spectral energy distributions (SEDs)
and compared them with radiative-transfer models developed by
\citet{Robitaille17}. Figure~7 in \citet{Azatyan19} shows examples of such
a comparison for the YSOs associated with IRAS sources in the IRAS 05168$+$3634
region.

%t1 #&#
\begin{table*}
\caption{The parameters of ISM and stellar population in the star-forming
regions}
\label{tab:par}
%%LEAP%%%\label{tab1}
%
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lllllllll@{}}
\hline%
\tmultirow{2}{*}{IRAS} & $\alpha $ (2000)  & $\delta $ (2000)  & N(H$_{2}$) & T$_{d}$  &
\tmultirow{2}{*}{YSOs} & Radius & D & A$_{v}$\\
 & (hh mm ss) & (dd mm ss)  & ($\times $ 10$^{23}$ cm$^{-2}$)  & (K)  &  & (pc) & (kpc) & (mag)\\
 \lcline{1-9}
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)\\
\bhline
05137$+$3919  & 05 17 13.3 & $+$39 22 14.0 & 0.25 $-$ 1.0 & 11 $-$ 22 & 33 & 1.9/4.8 & 4.4/11 & 1.8\\
[3pt]
05184$+$3635  & 05 21 53.2 & $+$36 38 20.4  & 1.1 $-$ 1.5  & 12 $-$ 15 & 52 & 1.4 & 1.9 & 1.4\\
05177$+$3636  & 05 21 09.4 & $+$36 39 37.1  & 1.1 $-$ 2.3   & 12 $-$ 13  & 79 & 1.9 & 1.9 & 1.3 \\
05168$+$3634  & 05 20 16.4 & $+$36 37 18.7  & 1.1 $-$ 3.8   & 11 $-$ 24 & 57 & 1.7 & 1.9 & 4.5\\
05162$+$3639  & 05 19 38.4 & $+$36 42 25.0 & 0.9 $-$ 1.0   & 11 $-$ 12  & 5 & 0.14 & 1.9 & 1.2\\
05156$+$3643  & 05 19 03.6 & $+$36 46 15.7 & 1.1 $-$ 1.6   & 11 $-$ 12  & 47 & 1.5 & 1.9 & 1.0\\
[3pt]
19110$+$1045 & 19 13 22.0 & $+$10 50 54.0 & 3.0 $-$ 5.0  & 18 $-$ 42 & 37 & 1.8 & 7.8 & 13\\
19111$+$1048 & 19 13 27.8 & $+$10 53 36.7 & 3.0 $-$ 5.5  & 18 $-$ 35 & 87 & 2.7 & 7.8 & 13\\
\hline
\end{tabular*}
\begin{tabnotes}
\legend{Note: (1) names of (sub-)regions, (2),(3) coordinates of the IRAS sources,
(4) ranges of hydrogen column density, (5) ranges of dust temperature, (6) numbers of
YSOs within the selected radii, (7) the radii of (sub-)regions, (8) adopted
distances of the regions, (9) the median interstellar extinctions estimated
with the SED fitting tool for IRAS 05137$+$3919 and 19110$+$1045 and 19111$+$1048
star-forming regions, and according to the COBE/DIRBE and IRAS/ISSA maps
\citep{Schlegel98} for the IRAS 05168$+$3634 star-forming region.}
\end{tabnotes}
\end{table*}

%s3 #&#
\section{Results and discussion}
%%LEAP%%%\label{sec3}
\label{3}

The selected regions (IRAS 05137$+$3919, 05168$+$3634, and 19110$+$1045), among
other things, hold particular interest due to their considerable distances,
providing an opportunity to evaluate the capabilities of the databases
we have access to. For the IRAS 05137$+$3919, the distance estimates based
on radio observations have a large variation: from $\sim $ 4.4 kpc
\citep{Casoli86,Wouterloot89} to 10.8 kpc \citep{Molinari96}. The distance
estimations of IRAS 05168$+$3634 star-forming region are also different:
6.08 kpc \citep{Molinari96} and $1.88^{+0.21}_{-0.17}$ kpc
\citep{Sakai12}. Given the significant discrepancy in the distance estimates
for the IRAS 05168$+$3634 star-forming region, we attempted to identify
YSOs within the \textit{Gaia} EDR3 database. The results obtained from
the \textit{Gaia} EDR3 data provide additional support to the fact that
this star-forming region is situated at a distance of $\sim $1.9 kpc
\citep{Nikoghosyan21}. Finally, the distance estimate for the IRAS 19110$+$1045
star-forming region is 7.75 $\pm $ 0.45 kpc \citep{Wu19}. Table~\ref{tab:par} contains the parameters of ISM and stellar population in
the star-forming regions and below are the results of their study.

%\singlespacing

In the vicinity of \textbf{IRAS 05137}$\boldsymbol{+}$\textbf{3919}, we observed a young stellar
cluster closely associated with the CPM 15 YSO \citep{Campbell89} (Fig.~\ref{fig:regions} top left). This region exhibits various signs of active
star formation, including maser emissions, as well as the presence of CO
and H$_{2}$ outflows \citep{Zhang05, Varricatt10}. The results of modified
single-temperature blackbody fitting are presented in (4) and (5) Columns
of Table~\ref{tab:par}. The maxima for both N(H$_{2}$) and T$_{d}$ coincide
with the position of the IRAS source. Within the determined 1.5\'  radius,
we identified 33 YSOs using two c--c diagrams. We were able to derive the
parameters of these YSOs using the SED fitting tool. These selected YSOs
exhibit a nonuniform distribution within the star-forming region, forming
two distinct subgroups. One of these subgroups is situated around CPM 15,
while the second group encompasses a notable number of middle-mass objects,
surrounded by gas-dust nebulae \citep{Nikoghosyan14}.

%\singlespacing

The next young stellar cluster is concentrated around the
\textbf{IRAS 05168}$\boldsymbol{+}$\textbf{3634} source. The presence of diverse maser emissions
and the existence of $^{13}$CO cores provide compelling evidence of its
ongoing star-forming activity \citep{Zhang05, Fontani10,Guan08}. Notably,
in the FIR wavelengths, the region exhibits a more intricate and complex
structure compared to its appearance in the NIR, as illustrated in the
bottom panel of Fig.~\ref{fig:regions}. Our investigation of the whole
star-forming region within the molecular cloud unveiled the presence of
four additional IRAS sources at the same distance, namely IRAS 05184$+$3635,
05177$+$3636, 05162$+$3639, and 05156$+$3643, which are embedded into a
$\sim $26 pc long cloud complex \citep{Azatyan19}. The results of modified
single-temperature blackbody fitting are presented in Table~\ref{tab:par} for each IRAS subregion. Notably, the relatively warmer gas-dusty
material leads to dense condensations around the IRAS objects
\citep{Nikoghosyan21}. An exception is the IRAS 05162$+$3639 subregion where
the N(H$_{2}$) map reveals a distinct absence of regions with relatively
higher density. Additionally, no cluster of YSOs has been identified around
this source; instead, only five stars are present. Within the determined
radii, we identify YSOs using four c--c diagrams and the results are presented
in (6) Column of Table~\ref{tab:par} for each IRAS subregion. Comprehensive
tables containing information on the selected YSOs, including their NIR,
MIR, and FIR photometry, as well as parameters obtained through the SED
fitting tool, can be accessed via the VizieR On-line Data Catalog\footnote{The
full tables are available in the VizieR On-line Data Catalog: J/A$+$A/622/A38.}
\citep{Azatyan19}.

%\singlespacing

The final star-forming region is associated with the
\textbf{IRAS 19110}$\boldsymbol{+}$\textbf{1045} and \textbf{19111}$\boldsymbol{+}$\textbf{1048} sources, which are commonly
referred to as the \textbf{G45.07}$\boldsymbol{+}$\textbf{0.13} and \textbf{G45.12}$\boldsymbol{+}$\textbf{0.13} UCHII regions,
respectively. This system serves as an ideal laboratory for the exploration
of the initial phases of massive star formation and their impact on their
surrounding environments. Figure~\ref{fig:regions}, top right panel, shows
a color-composite image of the region and it also indicates that these
UCHII regions are interconnected by a relatively cooler bridge, strongly
suggesting that they form a physically linked system. The results of modified
single-temperature blackbody fitting are presented in Table~\ref{tab:par} for each IRAS subregion. In the G45.07$+$0.13 region, the IRAS
source is slightly offset from the density peak, while in the G45.12$+$0.13
region, the position of IRAS 19111$+$1048 coincides with the maxima of both
T$_{d}$ and N(H$_{2}$). Let us note that in this star-forming region both
T$_{d}$ and N(H$_{2}$) are the highest. Within the determined radii, we
identify YSOs using six c--c diagrams and the results are presented in
Column (6) of Table~\ref{tab:par} for each IRAS subregion. As in the previous
cases, we included objects classified as YSOs in at least two c--c diagrams
in our list. However, due to the presence of two saturated areas in the
MIR band surrounding the IRAS sources (IRAS 19110$+$1045 with a 25$''$ radius
and IRAS 19111$+$1048 with a 50$''$ radius), objects within those regions
were classified as YSO candidates based solely on the NIR c--c diagram
and we conducted a visual inspection of the YSO candidates (95 YSOs) in
the two MIR-saturated regions, as these objects are of particular interest
due to their proximity to the UCHIIs. The comprehensive tables containing
information on the selected YSOs, including their NIR, MIR, and FIR photometry,
as well as parameters derived from the SED fitting tool, can be accessed
in the VizieR On-line Data Catalog.\footnote{The complete dataset is accessible
in the VizieR On-line Data Catalog: J/other/PASA/39.24.} Among the considered
three star-forming regions, massive stars were only detected in this one.
In the G45.07$+$0.13 region, we identified two massive stars, while in the
G45.12$+$0.13 region there were four, and one of them with a mass of 9.4{
\textpm}4.3 M$_{\odot}$, a temperature of 23 000 {\textpm}11 000~K,
and an evolutionary age of (2.5 {\textpm}1.2)x10$^{6}$ years was successfully
identified as the NIR counterpart of the IRAS 19111$+$1048 source
\citep{Azatyan22}.

%f3 #&#
\begin{figure}
\includegraphics{4298f03}
\caption{(\textit{Bottom}) K versus (J--K) CMDs for the identified YSOs in
the three star-forming regions. In this diagram, blue crosses represent
stellar objects in the IRAS 19110$+$1045 and 19111$+$1048 star-forming regions
labeled as IRAS 19110$+$1045, green circles represent objects located in
the IRAS 05137$+$3919 star-forming region, and finally yellow stars represent
stellar objects in the IRAS 05168$+$3634 star-forming region. The premain
sequence isochrones for the 0.1 and 1 Myr \citep{siess00} and ZAMS are
drawn as solid thin and thick lines, respectively. The positions of a few
spectral types are labeled. The J and K magnitudes of the YSOs are corrected
for the median interstellar extinctions and distances separately. The solid
arrow indicates the average slope of NIR excesses caused by circumstellar
discs \citep{lopez07}. (\textit{Top}) Histograms of (J--K)$_{abs}$ values
of the three star-forming regions with the same colors.}
\label{fig:cmd19110}
\end{figure}
%%LEAP%%%\label{fig3}


%f4 #&#
\begin{figure}
\includegraphics{4298f04}
\caption{Histograms of the evolutionary ages for members of the three star-forming
regions. The colors are the same as in Fig.~\protect\ref{fig:cmd19110}. The bin
size corresponds to Log (Age) $=$ 0.25.}
\label{fig:age}
\end{figure}
%%LEAP%%%\label{fig4}


%\singlespacing

Figure~\ref{fig:cmd19110}, bottom panel, shows the distribution of the
identified YSOs in the color--magnitude diagram (CMD). The correction of
J and K magnitudes of the YSOs for each region was done with the median
interstellar extinctions and the adopted distances taken from Table~\ref{tab:par}. For IRAS 05137$+$3919, we used only a 4.4 kpc distance.
The members of each star-forming regions are indicated with different colors
and symbols. As we can see, the members of each star-forming regions display
different dispersion concerning the isochrones (solid thin and thick lines).
The members in IRAS 05137$+$3919 and 05168$+$3634 star-forming regions show
large dispersion concerning the isochrones, while the members in IRAS 19110$+$1045
and 19111$+$1048 star-forming regions display relatively low dispersion concerning
the isochrones and they are more evolved. To enhance clarity, the histograms
for (J--K)$_{abs}$ are presented in the top panel with the same colors
as in the bottom panel. In general, the stellar objects in IRAS 05137$+$3919
and 05168$+$3634 star-forming regions, display large spreads in (J--K)$_{abs}$,
while the members in IRAS 19110$+$1045 and 19111$+$1048 star-forming regions
are mostly concentrated. For the comparison, we also constructed the histograms
of the evolutionary ages for the members of the star-forming regions based
on the results of the SED fitting tool. Figure~\ref{fig:age} presents histograms
of the evolutionary ages with the same colors as in Fig.~\ref{fig:cmd19110}. The histograms revealed a notably wide spread for all
regions. It should be noted that the evolutionary age distribution for
the objects in IRAS 19110$+$1045 and 19111$+$1048 star-forming regions (blue
bars) is derived from parameters obtained for only 29 YSOs subjected to
the SED fitting tool. Most of the remaining 95 YSOs within the MIR-saturated
regions are concentrated around the zero-age main sequence (ZAMS) and situated
to the left of the 1 Myr isochrone. Consequently, it is posited that these
objects significantly contribute to the first peak in the evolutionary
age distribution, rendering it a single, well-defined peak similar to the
(J--K)$_{abs}$ histogram. Consequently, the large age spread observed in
the IRAS 05137$+$3919 and 05168$+$3634 star-forming regions provides strong
evidence to support the conclusion that the stellar populations within
them are the outcome of independent condensations within the parent molecular
cloud. On the contrary, the small spread of evolutionary ages in IRAS 19110$+$1045
and 19111$+$1048 star-forming regions suggests that formation of the stellar
population may be attributed to a triggering shock. We assume that Granat
1915$+$105 High Mass X-ray Binary, which is located at the same distance
as IRAS 19110$+$1045 and 19111$+$1048 star-forming regions and belongs to
the same molecular cloud, could be the possible trigger of the star formation
in these regions. We plan to check the reliability of this assumption in
our future work.

%s4 #&#
\section{Conclusion}
%%LEAP%%%\label{sec4}
\label{4}

Here are the main findings from the detailed study of the IRAS 05137$+$3919,
05168$+$3634, 19110$+$1045 and 19111$+$1048 star-forming regions:
%
\begin{itemize}
%
\item A total of 33 YSOs were identified in the IRAS 05137$+$\noxml{\break}3919 region,
240 YSOs in the IRAS 05168$+$3634 region, and totally, 124 YSOs in the IRAS 19110$+$1045
and 19111$+$1048 regions.
%
\item In the IRAS 05137$+$3919 star-forming region, the selected YSOs are
not uniformly distributed and form two distinct subgroups.
%
\item In the IRAS 05168$+$3634 field, five dense subgroups were detected
around IRAS sources, indicating that IRAS 05168$+$3634 and four other subregions
are embedded into a $\sim $26 pc long cloud complex, located at a
$\sim $1.9 kpc distance based on \textit{Gaia} EDR3 parallax measurements.
%
\item Both IRAS 05137$+$3919 and IRAS 05168$+$3634 star-forming regions exhibit
a wide age spread, suggesting that the stellar populations within these
regions formed independently within the parent molecular clouds.
%
\item The members of the IRAS clusters in the G45.12$+$0.13 and G45.07$+$0.13
UC HII regions show low scatter relative to the isochrones, and their
age distribution indicates a small spread, possibly related to an external
triggering shock.
%
\item Among the considered star-forming regions, massive stars were only
detected in the region where star formation may have been triggered and
the temperature and hydrogen column density of the ISM are the highest,
specifically IRAS 19110$+$1045 and 19111$+$1048.
%
\end{itemize}
%
These findings provide valuable insights into the structure, formation,
and age distribution of stars within these star-forming regions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{backmatter}

%\begin{appendix}
%%\appsection*{Appendix:\enskip Title}
%\end{appendix}

%% break lines using \onlinebreak
%\begin{online}
%\ESM{}{}{}\label{}
%\ESM{}{}{}\label{}
%\end{online}

%\printesmhint

\begin{acks}
I thank the anonymous reviewer for
constructive comments and suggestions. I would like to thank my supervisor,
Dr. Elena Nikoghosyan, for her invaluable supervision and support during
the course of my PhD degree. This work partially was made possible by a
research grant number N0 21AG-1C044 from the Science Committee of Ministry
of Education, Science, Culture and Sports RA.
\end{acks}

\begin{authorcontribution}[Author contributions]% Updated by JobSheet2LaTeX.exe, 29.03.2024 09:35
N. A. prepared the manuscript.
\end{authorcontribution}

%\begin{fundinginformation}%[]
%\end{fundinginformation}

%\begin{dataavailability}%[]
%\end{dataavailability}

%\begin{materialsavailability}
%\end{materialsavailability}

%\begin{codeavailability}
%\end{codeavailability}

\begin{ethics}
%\begin{conflict}%[]
%\end{conflict}
\begin{competinginterests}[Competing interests]% Updated by JobSheet2LaTeX.exe, 29.03.2024 09:35
The authors declare no competing interests.
\end{competinginterests}
\end{ethics}
% structpyb loaded by imikolaityte, 2024-03-29 09:57:50
\begin{thebibliography}{}

%%% bbsrt2.pl, ver. 2.5.8, 2017.08.09
%b1 ###bbsrt2
%b1 ###
\bibitem[\protect\citeauthoryear{Ambartsumian}{1947}]{Ambartsumian47}
\begin{botherref}
\oauthor{\bsnm{Ambartsumian}, \binits{V.A.}}:
The evolution of stars and astrophysics
(\byear{1947})
\end{botherref}
\OrigBibText
Ambartsumian VA (1947) The evolution of stars and astrophysics
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b2 ###bbsrt2
%b4 ###
\bibitem[\protect\citeauthoryear{Azatyan}{2019}]{Azatyan19}
\begin{barticle}
\bauthor{\bsnm{Azatyan}, \binits{N.M.}}:
\batitle{Investigation of the stellar content in the IRAS 05168$+$3634 star-forming region}.
\bjtitle{Astron. Astrophys.}
\bvolume{622},
\bnumber{A38}
(\byear{2019}).
\doiurl{https://doi.org/10.1051/0004-6361/201731904}.
\bcomment{\arxivurl{1812.06808} [astro-ph.SR]}
\end{barticle}
\OrigBibText
Azatyan NM (2019) Investigation of the stellar content in the IRAS 05168$+$3634
star-forming region. Astronomy \& Astrophysics 622:A38.
\url{https://doi.org/10.1051/0004-6361/201731904}, arXiv:1812.06808
[astro-ph.SR]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b3 ###bbsrt2
%b5 ###
\bibitem[\protect\citeauthoryear{Azatyan and Nikoghosyan}{2018}]{Azatyan18}
\begin{barticle}
\bauthor{\bsnm{Azatyan}, \binits{N.M.}},
\bauthor{\bsnm{Nikoghosyan}, \binits{E.H.}}:
\batitle{Investigation of the stellar content in the IRAS 05168$+$3634 star-forming region}.
\bjtitle{Commun. Byurakan Astrophys. Obs.}
\bvolume{65}(\bissue{2}),
\bfpage{228}--\blpage{239}
(\byear{2018}).
\doiurl{https://doi.org/10.52526/25792776-2018.2.2-228}
\end{barticle}
\OrigBibText
Azatyan NM, Nikoghosyan EH (2018) Investigation of the stellar content
in the IRAS 05168$+$3634 star-forming region. Commun. Byurakan Astrophys. Obs. 65(2):228--239.
\url{https://doi.org/10.52526/25792776-2018.2.2-228}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b4 ###bbsrt2
%b6 ###
\bibitem[\protect\citeauthoryear{Azatyan et~al.}{2016}]{azatyan16}
\begin{barticle}
\bauthor{\bsnm{Azatyan}, \binits{N.M.}},
\bauthor{\bsnm{Nikoghosyan}, \binits{E.H.}},
\bauthor{\bsnm{Khachatryan}, \binits{K.G.}}:
\batitle{Search for compact stellar groups in the vicinity of iras sources}.
\bjtitle{Astrophysics}
\bvolume{59},
\bfpage{339}--\blpage{353}
(\byear{2016}).
\doiurl{https://doi.org/10.1007/s10511-016-9439-4}.
\bcomment{\arxivurl{1608.02225} [astro-ph.SR]}
\end{barticle}
\OrigBibText
Azatyan NM, Nikoghosyan EH, Khachatryan KG (2016) Search for Compact
Stellar Groups in the Vicinity of Iras Sources. \textit{Astrophysics}, \textbf{59}, 339--353.
\url{https://doi.org/10.1007/s10511-016-9439-4}, arXiv:1608.02225
[astro-ph.SR]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b5 ###bbsrt2
%b2 ###
\bibitem[\protect\citeauthoryear{Azatyan et~al.}{2020}]{Azatyan20}
\begin{barticle}
\bauthor{\bsnm{Azatyan}, \binits{N.}},
\bauthor{\bsnm{Nikoghosyan}, \binits{E.}},
\bauthor{\bsnm{Harutyunian}, \binits{H.}}, \betal:
\batitle{Stellar population in two star-forming regions}.
\bjtitle{Commun. Byurakan Astrophys. Obs.}
\bvolume{67},
\bfpage{211}--\blpage{218}
(\byear{2020}).
\doiurl{https://doi.org/10.52526/25792776-2020.67.2-211}
\end{barticle}
\OrigBibText
Azatyan N, Nikoghosyan E, Harutyunian H, et~al (2020) Stellar population
in two star-forming regions. Commun. Byurakan Astrophys. Obs. 67:211--218.
\url{https://doi.org/10.52526/25792776-2020.67.2-211}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b6 ###bbsrt2
%b3 ###
\bibitem[\protect\citeauthoryear{Azatyan et~al.}{2022}]{Azatyan22}
\begin{barticle}
\bauthor{\bsnm{Azatyan}, \binits{N.}},
\bauthor{\bsnm{Nikoghosyan}, \binits{E.}},
\bauthor{\bsnm{Harutyunian}, \binits{H.}}, \betal:
\batitle{Infrared study of the star-forming region associated with the
UC HII regions G45.07$+$0.13 and G45.12$+$0.13}.
\bjtitle{Publ. Astron. Soc. Aust.}
\bvolume{39},
\bnumber{e024}
(\byear{2022}).
\doiurl{https://doi.org/10.1017/pasa.2022.20},
\bcomment{\arxivurl{2204.06338} [astro-ph.SR]}
\end{barticle}
\OrigBibText
Azatyan N, Nikoghosyan E, Harutyunian H, et~al (2022) Infrared study
of the star-forming region associated with the UC HII regions G45.07$+$0.13
and G45.12$+$0.13. \textit{Publ Astron Soc Aust}, \textbf{39}, e024.
\url{https://doi.org/10.1017/pasa.2022.20}, arXiv:2204.06338
[astro-ph.SR]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b7 ###bbsrt2
%b7 ###
\bibitem[\protect\citeauthoryear{Battersby et~al.}{2011}]{Battersby11}
\begin{barticle}
\bauthor{\bsnm{Battersby}, \binits{C.}},
\bauthor{\bsnm{Bally}, \binits{J.}},
\bauthor{\bsnm{Ginsburg}, \binits{A.}}, \betal:
\batitle{Characterizing precursors to stellar clusters with Herschel}.
\bjtitle{Astron. Astrophys.}
\bvolume{535},
\bnumber{A128}
(\byear{2011}).
\doiurl{https://doi.org/10.1051/0004-6361/201116559}.
\bcomment{\arxivurl{1101.4654} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Battersby C, Bally J, Ginsburg A, et~al (2011) Characterizing precursors
to stellar clusters with Herschel. Astronomy \& Astrophysics 535:A128.
\url{https://doi.org/10.1051/0004-6361/201116559}, arXiv:1101.4654
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b8 ###bbsrt2
%b8 ###
\bibitem[\protect\citeauthoryear{Campbell et~al.}{1989}]{Campbell89}
\begin{barticle}
\bauthor{\bsnm{Campbell}, \binits{B.}},
\bauthor{\bsnm{Persson}, \binits{S.E.}},
\bauthor{\bsnm{Matthews}, \binits{K.}}:
\batitle{Identifications of new young stellar objects associated with
IRAS point sources. III. The northern galactic plane}.
\bjtitle{Astron. J.}
\bvolume{98},
\bfpage{643}
(\byear{1989}).
\doiurl{https://doi.org/10.1086/115164}
\end{barticle}
\OrigBibText
Campbell B, Persson SE, Matthews K (1989) Identifications of New
Young Stellar Objects Associated with IRAS Point Sources. III. The Northern
Galactic Plane. \textit{Astronomical Journal} \textbf{98}, 643.
\url{https://doi.org/10.1086/115164}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b9 ###bbsrt2
%b9 ###
\bibitem[\protect\citeauthoryear{Carey et~al.}{2009}]{Carey09}
\begin{barticle}
\bauthor{\bsnm{Carey}, \binits{S.J.}},
\bauthor{\bsnm{Noriega-Crespo}, \binits{A.}},
\bauthor{\bsnm{Mizuno}, \binits{D.R.}}, \betal:
\batitle{MIPSGAL: a survey of the inner galactic plane at 24 and 70 \textmu m}.
\bjtitle{Publ. Astron. Soc. Pac.}
\bvolume{121}(\bissue{875}),
\bfpage{76}
(\byear{2009}).
\doiurl{https://doi.org/10.1086/596581}
\end{barticle}
\OrigBibText
Carey SJ, Noriega-Crespo A, Mizuno DR, et~al (2009) MIPSGAL: A Survey
of the Inner Galactic Plane at 24 and 70~\textmu m. Publ Astron
Soc Pac 121(875):76. \url{https://doi.org/10.1086/596581}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b10 ###bbsrt2
%b10 ###
\bibitem[\protect\citeauthoryear{Casoli et~al.}{1986}]{Casoli86}
\begin{barticle}
\bauthor{\bsnm{Casoli}, \binits{F.}},
\bauthor{\bsnm{Dupraz}, \binits{C.}},
\bauthor{\bsnm{Gerin}, \binits{M.}}, \betal:
\batitle{13CO and 12CO observations of cold IRAS unidentified point sources inthe galaxy}.
\bjtitle{Astron. Astrophys.}
\bvolume{169},
\bfpage{281}--\blpage{297}
(\byear{1986})
\end{barticle}
\OrigBibText
Casoli F, Dupraz C, Gerin M, et~al (1986) 13CO and 12CO observations
of cold IRAS unidentified point sources inthe galaxy. Astronomy \& Astrophysics
169:281--297
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b11 ###bbsrt2
%b11 ###
\bibitem[\protect\citeauthoryear{Churchwell et~al.}{2009}]{churchwell09}
\begin{barticle}
\bauthor{\bsnm{Churchwell}, \binits{E.}},
\bauthor{\bsnm{Babler}, \binits{B.L.}},
\bauthor{\bsnm{Meade}, \binits{M.R.}}, \betal:
\batitle{The Spitzer/GLIMPSE surveys: a new view of the Milky Way}.
\bjtitle{Publ. Astron. Soc. Pac.}
\bvolume{121},
\bfpage{213}--\blpage{230}
(\byear{2009}).
\doiurl{https://doi.org/10.1086/597811}
\end{barticle}
\OrigBibText
Churchwell E, Babler BL, Meade MR, et~al (2009) The Spitzer/GLIMPSE
Surveys: A New View of the Milky Way. \textit{Publ Astron Soc Pac} \textbf{121}, 213--230.
\url{https://doi.org/10.1086/597811}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b12 ###bbsrt2
%b12 ###
\bibitem[\protect\citeauthoryear{Cutri et~al.}{2003}]{Cutri03}
\begin{bbook}
\bauthor{\bsnm{Cutri}, \binits{R.M.}},
\bauthor{\bsnm{Skrutskie}, \binits{M.F.}},
\bauthor{\bparticle{van} \bsnm{Dyk}, \binits{S.}}, \betal:
\bbtitle{VizieR Online Data Catalog: 2MASS All-Sky Catalog of Point Sources
(Cutri$+$ 2003). VizieR Online Data Catalog II/246}
(\byear{2003})
\end{bbook}
\OrigBibText
Cutri R.M., Skrutskie M.F., van Dyk S., et~al (2003) VizieR Online Data
Catalog: 2MASS All-Sky Catalog of Point Sources (Cutri$+$ 2003). VizieR
Online Data Catalog II/246
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b13 ###bbsrt2
%b13 ###
\bibitem[\protect\citeauthoryear{Fontani et~al.}{2010}]{Fontani10}
\begin{barticle}
\bauthor{\bsnm{Fontani}, \binits{F.}},
\bauthor{\bsnm{Cesaroni}, \binits{R.}},
\bauthor{\bsnm{Furuya}, \binits{R.S.}}:
\batitle{Class I and Class II methanol masers in high-mass star-forming regions}.
\bjtitle{Astron. Astrophys.}
\bvolume{517},
\bnumber{A56}
(\byear{2010}).
\doiurl{https://doi.org/10.1051/0004-6361/200913679}.
\bcomment{\arxivurl{1004.3689} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Fontani F, Cesaroni R, Furuya RS (2010) Class I and Class II methanol
masers in high-mass star-forming regions. Astronomy \& Astrophysics 517:A56.
\url{https://doi.org/10.1051/0004-6361/200913679}, arXiv:1004.3689
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b14 ###bbsrt2
%b14 ###
\bibitem[\protect\citeauthoryear{Griffin et~al.}{2010}]{griffin10}
\begin{barticle}
\bauthor{\bsnm{Griffin}, \binits{M.J.}},
\bauthor{\bsnm{Abergel}, \binits{A.}},
\bauthor{\bsnm{Abreu}, \binits{A.}}, \betal:
\batitle{The Herschel-SPIRE instrument and its in-flight performance}.
\bjtitle{Astron. Astrophys.}
\bvolume{518},
\bnumber{L3}
(\byear{2010}).
\doiurl{https://doi.org/10.1051/0004-6361/201014519}.
\bcomment{\arxivurl{1005.5123} [astro-ph.IM]}
\end{barticle}
\OrigBibText
Griffin MJ, Abergel A, Abreu A, et~al (2010) The Herschel-SPIRE
instrument and its in-flight performance. Astronomy \& Astrophysics 518:L3.
\url{https://doi.org/10.1051/0004-6361/201014519}, arXiv:1005.5123
[astro-ph.IM]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b15 ###bbsrt2
%b15 ###
\bibitem[\protect\citeauthoryear{Guan et~al.}{2008}]{Guan08}
\begin{barticle}
\bauthor{\bsnm{Guan}, \binits{X.}},
\bauthor{\bsnm{Wu}, \binits{Y.}},
\bauthor{\bsnm{Ju}, \binits{B.}}:
\batitle{A mapping survey of massive CO cores}.
\bjtitle{Mon. Not. R. Astron. Soc.}
\bvolume{391}(\bissue{2}),
\bfpage{869}--\blpage{880}
(\byear{2008}).
\doiurl{https://doi.org/10.1111/j.1365-2966.2008.13937.x}
\end{barticle}
\OrigBibText
Guan X, Wu Y, Ju B (2008) A mapping survey of massive CO cores.
Mon Not R Astron Soc 391(2):869--880.
\url{https://doi.org/10.1111/j.1365-2966.2008.13937.x}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b16 ###bbsrt2
%b16 ###
\bibitem[\protect\citeauthoryear{Hildebrand}{1983}]{hildebrand83}
\begin{barticle}
\bauthor{\bsnm{Hildebrand}, \binits{R.H.}}:
\batitle{The determination of cloud masses and dust characteristics from
submillimetre thermal emission}.
\bjtitle{Q. J. R. Astron. Soc.}
\bvolume{24},
\bfpage{267}--\blpage{282}
(\byear{1983})
\end{barticle}
\OrigBibText
Hildebrand RH (1983) The determination of cloud masses and dust characteristics
from submillimetre thermal emission. QJRAS 24:267--282
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b17 ###bbsrt2
%b17 ###
\bibitem[\protect\citeauthoryear{Kauffmann et~al.}{2008}]{Kauffmann08}
\begin{barticle}
\bauthor{\bsnm{Kauffmann}, \binits{J.}},
\bauthor{\bsnm{Bertoldi}, \binits{F.}},
\bauthor{\bsnm{Bourke}, \binits{T.L.}}, \betal:
\batitle{MAMBO mapping of Spitzer c2d small clouds and cores}.
\bjtitle{Astron. Astrophys.}
\bvolume{487}(\bissue{3}),
\bfpage{993}--\blpage{1017}
(\byear{2008}).
\doiurl{https://doi.org/10.1051/0004-6361:200809481}.
\bcomment{\arxivurl{0805.4205} [astro-ph]}
\end{barticle}
\OrigBibText
Kauffmann J, Bertoldi F, Bourke TL, et~al (2008) MAMBO mapping of
Spitzer c2d small clouds and cores. Astronomy \& Astrophysics 487(3):993--1017.
\url{https://doi.org/10.1051/0004-6361:200809481}, arXiv:0805.4205
[astro-ph]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b18 ###bbsrt2
%b18 ###
\bibitem[\protect\citeauthoryear{K\"{o}nyves et~al.}{2015}]{Konyves15}
\begin{barticle}
\bauthor{\bsnm{K\"{o}nyves}, \binits{V.}},
\bauthor{\bsnm{Andr\'{e}}, \binits{P.}},
\bauthor{\bsnm{Men'shchikov}, \binits{A.}}, \betal:
\batitle{A census of dense cores in the Aquila cloud complex: SPIRE/PACS
observations from the Herschel Gould Belt survey}.
\bjtitle{Astron. Astrophys.}
\bvolume{584},
\bnumber{A91}
(\byear{2015}).
\doiurl{https://doi.org/10.1051/0004-6361/201525861}.
\bcomment{\arxivurl{1507.05926} [astro-ph.GA]}
\end{barticle}
\OrigBibText
K\"onyves V., Andr\'e P., Men'shchikov A., et~al (2015) A census
of dense cores in the Aquila cloud complex: SPIRE/PACS observations from
the Herschel Gould Belt survey. \textit{Astronomy \& Astrophysics} \textbf{584}, A91.
\url{https://doi.org/10.1051/0004-6361/201525861}, arXiv:1507.05926
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b19 ###bbsrt2
%b19 ###
\bibitem[\protect\citeauthoryear{Lada and Lada}{2003}]{lada03}
\begin{barticle}
\bauthor{\bsnm{Lada}, \binits{C.J.}},
\bauthor{\bsnm{Lada}, \binits{E.A.}}:
\batitle{Embedded clusters in molecular clouds}.
\bjtitle{Annu. Rev. Astron. Astrophys.}
\bvolume{41},
\bfpage{57}--\blpage{115}
(\byear{2003}).
\doiurl{https://doi.org/10.1146/annurev.astro.41.011802.094844}.
\bcomment{\arxivurl{astro-ph/0301540}}
\end{barticle}
\OrigBibText
Lada CJ, Lada EA (2003) Embedded Clusters in Molecular Clouds. \textit{Ann
Rev Astron Astrophys} \textbf{41}, 57--115.
\url{https://doi.org/10.1146/annurev.astro.41.011802.094844}, astro-ph/0301540
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b20 ###bbsrt2
%b20 ###
\bibitem[\protect\citeauthoryear{L\'{o}pez-Chico and Salas}{2007}]{lopez07}
\begin{barticle}
\bauthor{\bsnm{L\'{o}pez-Chico}, \binits{T.}},
\bauthor{\bsnm{Salas}, \binits{L.}}:
\batitle{Mass determination for T Tauri stars from JHK photometry}.
\bjtitle{Rev. Mex. Astron. Astrof\'{\i}s.}
\bvolume{43},
\bfpage{155}--\blpage{171}
(\byear{2007}).
\bcomment{\arxivurl{astro-ph/0611721}}
\end{barticle}
\OrigBibText
L\'opez-Chico T, Salas L (2007) Mass determination for T Tauri stars
from JHK Photometry. Rev Mex Astron Astrofis 43:155--171. astro-ph/0611721
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b21 ###bbsrt2
%b21 ###
\bibitem[\protect\citeauthoryear{Lucas et~al.}{2008}]{lucas08}
\begin{barticle}
\bauthor{\bsnm{Lucas}, \binits{P.W.}},
\bauthor{\bsnm{Hoare}, \binits{M.G.}},
\bauthor{\bsnm{Longmore}, \binits{A.}}, \betal:
\batitle{The UKIDSS galactic plane survey}.
\bjtitle{Mon. Not. R. Astron. Soc.}
\bvolume{391},
\bfpage{136}--\blpage{163}
(\byear{2008}).
\doiurl{https://doi.org/10.1111/j.1365-2966.2008.13924.x}.
\bcomment{\arxivurl{0712.0100}}
\end{barticle}
\OrigBibText
Lucas PW, Hoare MG, Longmore A, et~al (2008) The UKIDSS Galactic
Plane Survey. \textit{Mon Not R Astron Soc} \textbf{391}, 136--163.
\url{https://doi.org/10.1111/j.1365-2966.2008.13924.x}, arXiv:0712.0100
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b22 ###bbsrt2
%b22 ###
\bibitem[\protect\citeauthoryear{Molinari et~al.}{1996}]{Molinari96}
\begin{barticle}
\bauthor{\bsnm{Molinari}, \binits{S.}},
\bauthor{\bsnm{Brand}, \binits{J.}},
\bauthor{\bsnm{Cesaroni}, \binits{R.}}, \betal:
\batitle{A search for precursors of ultracompact HII regions in a sample
of luminous IRAS sources. I. Association with ammonia cores}.
\bjtitle{Astron. Astrophys.}
\bvolume{308},
\bfpage{573}--\blpage{587}
(\byear{1996})
\end{barticle}
\OrigBibText
Molinari S, Brand J, Cesaroni R, et~al (1996) A search for precursors
of ultracompact HII regions in a sample of luminous IRAS sources. I. Association
with ammonia cores. Astronomy \& Astrophysics 308:573--587
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b23 ###bbsrt2
%b23 ###
\bibitem[\protect\citeauthoryear{Molinari et~al.}{2016}]{molinari16}
\begin{barticle}
\bauthor{\bsnm{Molinari}, \binits{S.}},
\bauthor{\bsnm{Schisano}, \binits{E.}},
\bauthor{\bsnm{Elia}, \binits{D.}}, \betal:
\batitle{Hi-GAL, the Herschel infrared Galactic Plane Survey: photometric
maps and compact source catalogues. First data release for the
inner Milky Way: $+$68{\textdegree} $\geq l \geq-70${\textdegree}}.
\bjtitle{Astron. Astrophys.}
\bvolume{591},
\bnumber{A149}
(\byear{2016}).
\doiurl{https://doi.org/10.1051/0004-6361/201526380}.
\bcomment{\arxivurl{1604.05911} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Molinari S, Schisano E, Elia D, et~al (2016) Hi-GAL, the Herschel
infrared Galactic Plane Survey: photometric maps and compact source catalogues.
First data release for the inner Milky Way: $+$68{\textdegree} $\geq$
l $\geq-$70{\textdegree}. Astronomy \& Astrophysics 591:A149.
\url{https://doi.org/10.1051/0004-6361/201526380}, arXiv:1604.05911
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b24 ###bbsrt2
%b24 ###
\bibitem[\protect\citeauthoryear{Neugebauer et~al.}{1984}]{Neugebauer84}
\begin{barticle}
\bauthor{\bsnm{Neugebauer}, \binits{G.}},
\bauthor{\bsnm{Habing}, \binits{H.J.}},
\bauthor{\bparticle{van} \bsnm{Duinen}, \binits{R.}}, \betal:
\batitle{The Infrared Astronomical Satellite (IRAS) mission}.
\bjtitle{Astrophys. J.}
\bvolume{278},
\bfpage{L1}--\blpage{L6}
(\byear{1984}).
\doiurl{https://doi.org/10.1086/184209}
\end{barticle}
\OrigBibText
Neugebauer G., Habing H.J., van Duinen R., et~al (1984) The Infrared
Astronomical Satellite (IRAS) mission. \textit{Astrophysical Journal} \textbf{278}, L1--L6.
\url{https://doi.org/10.1086/184209}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b25 ###bbsrt2
%b26 ###
\bibitem[\protect\citeauthoryear{Nikoghosyan and Azatyan}{2014}]{Nikoghosyan14}
\begin{barticle}
\bauthor{\bsnm{Nikoghosyan}, \binits{E.H.}},
\bauthor{\bsnm{Azatyan}, \binits{N.}}:
\batitle{Young stellar cluster in the vicinity of the IRAS 05137$+$3919 source}.
\bjtitle{Astrophysics}
\bvolume{57}(\bissue{3}),
\bfpage{330}--\blpage{343}
(\byear{2014}).
\doiurl{https://doi.org/10.1007/s10511-014-9338-5}
\end{barticle}
\OrigBibText
Nikoghosyan EH, Azatyan N (2014) Young Stellar Cluster in the Vicinity
of the IRAS 05137$+$3919 Source. Astrophysics 57(3):330--343.
\url{https://doi.org/10.1007/s10511-014-9338-5}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b26 ###bbsrt2
%b25 ###
\bibitem[\protect\citeauthoryear{Nikoghosyan et~al.}{2020}]{Nikoghosyan20}
\begin{barticle}
\bauthor{\bsnm{Nikoghosyan}, \binits{E.}},
\bauthor{\bsnm{Azatyan}, \binits{N.}},
\bauthor{\bsnm{Harutyunian}, \binits{H.}}, \betal:
\batitle{Properties of ISM in two star-forming regions}.
\bjtitle{Commun. Byurakan Astrophys. Obs.}
\bvolume{67},
\bfpage{187}--\blpage{192}
(\byear{2020}).
\doiurl{https://doi.org/10.52526/25792776-2020.67.2-187}
\end{barticle}
\OrigBibText
Nikoghosyan E, Azatyan N, Harutyunian H, et~al (2020) Properties
of ISM in two star-forming regions. Commun. Byurakan Astrophys. Obs. 67:187--192.
\url{https://doi.org/10.52526/25792776-2020.67.2-187}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b27 ###bbsrt2
%b27 ###
\bibitem[\protect\citeauthoryear{Nikoghosyan et~al.}{2021}]{Nikoghosyan21}
\begin{barticle}
\bauthor{\bsnm{Nikoghosyan}, \binits{E.H.}},
\bauthor{\bsnm{Azatyan}, \binits{N.M.}},
\bauthor{\bsnm{Andreasyan}, \binits{D.H.}}, \betal:
\batitle{The structure of the IRAS05168$+$3634 star-forming region}.
\bjtitle{Astrophys. Space Sci.}
\bvolume{366}(\bissue{11}),
\bfpage{114}
(\byear{2021}).
\doiurl{https://doi.org/10.1007/s10509-021-04023-4}.
\bcomment{\arxivurl{2111.02906} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Nikoghosyan EH, Azatyan NM, Andreasyan DH, et~al (2021) The structure
of the IRAS05168$+$3634 star-forming region. Astrophys Space Sci 366(11):114.
\url{https://doi.org/10.1007/s10509-021-04023-4}, arXiv:2111.02906
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b28 ###bbsrt2
%b28 ###
\bibitem[\protect\citeauthoryear{Pezzuto et~al.}{2021}]{pezzuto2021}
\begin{barticle}
\bauthor{\bsnm{Pezzuto}, \binits{S.}},
\bauthor{\bsnm{Benedettini}, \binits{M.}},
\bauthor{\bparticle{Di} \bsnm{Francesco}, \binits{J.}}, \betal:
\batitle{Physical properties of the ambient medium and of dense cores
in the Perseus star-forming region derived from Herschel Gould Belt Survey observations}.
\bjtitle{Astron. Astrophys.}
\bvolume{645},
\bnumber{A55}
(\byear{2021}).
\doiurl{https://doi.org/10.1051/0004-6361/201936534}.
\bcomment{\arxivurl{2010.00006} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Pezzuto S, Benedettini M, Di Francesco J, et~al (2021) Physical
properties of the ambient medium and of dense cores in the Perseus star-forming
region derived from Herschel Gould Belt Survey observations. Astronomy
\& Astrophysics 645:A55.
\url{https://doi.org/10.1051/0004-6361/201936534}, arXiv:2010.00006
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b29 ###bbsrt2
%b29 ###
\bibitem[\protect\citeauthoryear{Poglitsch et~al.}{2010}]{poglitsch10}
\begin{barticle}
\bauthor{\bsnm{Poglitsch}, \binits{A.}},
\bauthor{\bsnm{Waelkens}, \binits{C.}},
\bauthor{\bsnm{Geis}, \binits{N.}}, \betal:
\batitle{The Photodetector Array Camera and Spectrometer (PACS) on the Herschel space observatory}.
\bjtitle{Astron. Astrophys.}
\bvolume{518},
\bnumber{L2}
(\byear{2010}).
\doiurl{https://doi.org/10.1051/0004-6361/201014535}.
\bcomment{\arxivurl{1005.1487} [astro-ph.IM]}
\end{barticle}
\OrigBibText
Poglitsch A, Waelkens C, Geis N, et~al (2010) The Photodetector
Array Camera and Spectrometer (PACS) on the Herschel Space Observatory.
Astronomy \& Astrophysics 518:L2.
\url{https://doi.org/10.1051/0004-6361/201014535}, arXiv:1005.1487
[astro-ph.IM]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b30 ###bbsrt2
%b30 ###
\bibitem[\protect\citeauthoryear{Preibisch}{2012}]{Preibisch12}
\begin{barticle}
\bauthor{\bsnm{Preibisch}, \binits{T.}}:
\batitle{The reliability of age measurements for young stellar objects
from Hertzsprung-Russell or color-magnitude diagrams}.
\bjtitle{Res. Astron. Astrophys.}
\bvolume{12},
\bfpage{1}--\blpage{25}
(\byear{2012}).
\doiurl{https://doi.org/10.1088/1674-4527/12/1/001}
\end{barticle}
\OrigBibText
Preibisch T (2012) The reliability of age measurements for Young Stellar
Objects from Hertzsprung-Russell or color-magnitude diagrams. \textit{Research
in Astronomy and Astrophysics} \textbf{12}, 1--25.
\url{https://doi.org/10.1088/1674-4527/12/1/001}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b31 ###bbsrt2
%b31 ###
\bibitem[\protect\citeauthoryear{Price et~al.}{2001}]{Price01}
\begin{barticle}
\bauthor{\bsnm{Price}, \binits{S.D.}},
\bauthor{\bsnm{Egan}, \binits{M.P.}},
\bauthor{\bsnm{Carey}, \binits{S.J.}}, \betal:
\batitle{Midcourse space experiment survey of the galactic plane}.
\bjtitle{Astron. J.}
\bvolume{121}(\bissue{5}),
\bfpage{2819}--\blpage{2842}
(\byear{2001}).
\doiurl{https://doi.org/10.1086/320404}
\end{barticle}
\OrigBibText
Price SD, Egan MP, Carey SJ, et~al (2001) Midcourse Space Experiment
Survey of the Galactic Plane. Astronomical Journal 121(5):2819--2842.
\url{https://doi.org/10.1086/320404}
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b32 ###bbsrt2
%b32 ###
\bibitem[\protect\citeauthoryear{Robitaille}{2017}]{Robitaille17}
\begin{barticle}
\bauthor{\bsnm{Robitaille}, \binits{T.P.}}:
\batitle{A modular set of synthetic spectral energy distributions for young stellar objects}.
\bjtitle{Astron. Astrophys.}
\bvolume{600},
\bnumber{A11}
(\byear{2017}).
\doiurl{https://doi.org/10.1051/0004-6361/201425486}.
\bcomment{\arxivurl{1703.05765} [astro-ph.SR]}
\end{barticle}
\OrigBibText
Robitaille TP (2017) A modular set of synthetic spectral energy distributions
for young stellar objects. Astronomy \& Astrophysics 600:A11.
\url{https://doi.org/10.1051/0004-6361/201425486}, arXiv:1703.05765
[astro-ph.SR]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b33 ###bbsrt2
%b33 ###
\bibitem[\protect\citeauthoryear{Roy et~al.}{2014}]{roy2014}
\begin{barticle}
\bauthor{\bsnm{Roy}, \binits{A.}},
\bauthor{\bsnm{Andr\'{e}}, \binits{P.}},
\bauthor{\bsnm{Palmeirim}, \binits{P.}}, \betal:
\batitle{Reconstructing the density and temperature structure of prestellar
cores from Herschel data: a case study for B68 and L1689B}.
\bjtitle{Astron. Astrophys.}
\bvolume{562},
\bnumber{A138}
(\byear{2014}).
\doiurl{https://doi.org/10.1051/0004-6361/201322236}.
\bcomment{\arxivurl{1311.5086} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Roy A, Andr\'e P, Palmeirim P, et~al (2014) Reconstructing the
density and temperature structure of prestellar cores from Herschel data:
A case study for B68 and L1689B. Astronomy \& Astrophysics 562:A138.
\url{https://doi.org/10.1051/0004-6361/201322236}, arXiv:1311.5086
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b34 ###bbsrt2
%b34 ###
\bibitem[\protect\citeauthoryear{Sakai et~al.}{2012}]{Sakai12}
\begin{barticle}
\bauthor{\bsnm{Sakai}, \binits{N.}},
\bauthor{\bsnm{Honma}, \binits{M.}},
\bauthor{\bsnm{Nakanishi}, \binits{H.}}, \betal:
\batitle{Outer rotation curve of the galaxy with VERA I: trigonometric
parallax of IRAS 05168$+$3634}.
\bjtitle{Publ. Astron. Soc. Jpn.}
\bvolume{64},
\bfpage{108}
(\byear{2012}).
\doiurl{https://doi.org/10.1093/pasj/64.5.108}.
\bcomment{\arxivurl{1204.4782} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Sakai N, Honma M, Nakanishi H, et~al (2012) Outer Rotation Curve
of the Galaxy with VERA I: Trigonometric Parallax of IRAS 05168$+$3634.
Publ Astr Soc Japan 64:108.
\url{https://doi.org/10.1093/pasj/64.5.108}, arXiv:1204.4782
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b35 ###bbsrt2
%b35 ###
\bibitem[\protect\citeauthoryear{Schlegel et~al.}{1998}]{Schlegel98}
\begin{barticle}
\bauthor{\bsnm{Schlegel}, \binits{D.J.}},
\bauthor{\bsnm{Finkbeiner}, \binits{D.P.}},
\bauthor{\bsnm{Davis}, \binits{M.}}:
\batitle{Maps of dust infrared emission for use in estimation of reddening
and cosmic microwave background radiation foregrounds}.
\bjtitle{Astrophys. J.}
\bvolume{500}(\bissue{2}),
\bfpage{525}--\blpage{553}
(\byear{1998}).
\doiurl{https://doi.org/10.1086/305772}.
\bcomment{\arxivurl{astro-ph/9710327} [astro-ph]}
\end{barticle}
\OrigBibText
Schlegel D.J., Finkbeiner D.P., Davis M .(1998) Maps of Dust Infrared
Emission for Use in Estimation of Reddening and Cosmic Microwave Background
Radiation Foregrounds. \textit{Astrophysical Journal} \textbf{500}(2):525--553.
\url{https://doi.org/10.1086/305772}, arXiv:astro-ph/9710327
[astro-ph]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b36 ###bbsrt2
%b36 ###
\bibitem[\protect\citeauthoryear{Siess et~al.}{2000}]{siess00}
\begin{barticle}
\bauthor{\bsnm{Siess}, \binits{L.}},
\bauthor{\bsnm{Dufour}, \binits{E.}},
\bauthor{\bsnm{Forestini}, \binits{M.}}:
\batitle{An Internet server for pre-main sequence tracks of low- and intermediate-mass stars}.
\bjtitle{Astron. Astrophys.}
\bvolume{358},
\bfpage{593}--\blpage{599}
(\byear{2000}).
\bcomment{\arxivurl{astro-ph/0003477}}
\end{barticle}
\OrigBibText
Siess L, Dufour E, Forestini M (2000) An internet server for pre-main
sequence tracks of low- and intermediate-mass stars. Astronomy \& Astrophysics
358:593--599. astro-ph/0003477
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b37 ###bbsrt2
%b37 ###
\bibitem[\protect\citeauthoryear{Soderblom}{2010}]{Soderblom10}
\begin{barticle}
\bauthor{\bsnm{Soderblom}, \binits{D.R.}}:
\batitle{The ages of stars}.
\bjtitle{Annu. Rev. Astron. Astrophys.}
\bvolume{48},
\bfpage{581}--\blpage{629}
(\byear{2010}).
\doiurl{https://doi.org/10.1146/annurev-astro-081309-130806}.
\bcomment{\arxivurl{1003.6074} [astro-ph.SR]}
\end{barticle}
\OrigBibText
Soderblom DR (2010) The Ages of Stars. Ann Rev Astron Astrophys 48:581--629.
\url{https://doi.org/10.1146/annurev-astro-081309-130806}, arXiv:1003.6074
[astro-ph.SR]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b38 ###bbsrt2
%b38 ###
\bibitem[\protect\citeauthoryear{Varricatt et~al.}{2010}]{Varricatt10}
\begin{barticle}
\bauthor{\bsnm{Varricatt}, \binits{W.P.}},
\bauthor{\bsnm{Davis}, \binits{C.J.}},
\bauthor{\bsnm{Ramsay}, \binits{S.}}, \betal:
\batitle{A near-IR imaging survey of intermediate- and high-mass young stellar outflow candidates}.
\bjtitle{Mon. Not. R. Astron. Soc.}
\bvolume{404}(\bissue{2}),
\bfpage{661}--\blpage{720}
(\byear{2010}).
\doiurl{https://doi.org/10.1111/j.1365-2966.2010.16356.x}.
\bcomment{\arxivurl{1001.2708} [astro-ph.SR]}
\end{barticle}
\OrigBibText
Varricatt WP, Davis CJ, Ramsay S, et~al (2010) A near-IR imaging
survey of intermediate- and high-mass young stellar outflow candidates.
Mon Not R Astron Soc 404(2):661--720.
\url{https://doi.org/10.1111/j.1365-2966.2010.16356.x}, arXiv:1001.2708
[astro-ph.SR]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b39 ###bbsrt2
%b39 ###
\bibitem[\protect\citeauthoryear{Wouterloot and Brand}{1989}]{Wouterloot89}
\begin{barticle}
\bauthor{\bsnm{Wouterloot}, \binits{J.G.A.}},
\bauthor{\bsnm{Brand}, \binits{J.}}:
\batitle{IRAS sources beyond the solar circle. I. CO observations}.
\bjtitle{Astron. Astrophys. Suppl. Ser.}
\bvolume{80},
\bfpage{149}--\blpage{187}
(\byear{1989})
\end{barticle}
\OrigBibText
Wouterloot JGA, Brand J (1989) IRAS sources beyond the solar circle.
I. CO observations. Astronomy and Astrophysics Suppl Ser 80:149--187
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b40 ###bbsrt2
%b40 ###
\bibitem[\protect\citeauthoryear{Wright et~al.}{2010}]{wright10}
\begin{barticle}
\bauthor{\bsnm{Wright}, \binits{E.L.}},
\bauthor{\bsnm{Eisenhardt}, \binits{P.R.M.}},
\bauthor{\bsnm{Mainzer}, \binits{A.K.}}, \betal:
\batitle{The Wide-field Infrared Survey Explorer (WISE): mission description
and initial on-orbit performance}.
\bjtitle{Astron. J.}
\bvolume{140},
\bfpage{1868}--\blpage{1881}
(\byear{2010}).
\doiurl{https://doi.org/10.1088/0004-6256/140/6/1868}.
\bcomment{\arxivurl{1008.0031} [astro-ph.IM]}
\end{barticle}
\OrigBibText
Wright EL, Eisenhardt PRM, Mainzer AK, et~al (2010) The Wide-field
Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit
Performance. Astronomical Journal 140:1868-1881.
\url{https://doi.org/10.1088/0004-6256/140/6/1868}, arXiv:1008.0031
[astro-ph.IM]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b41 ###bbsrt2
%b41 ###
\bibitem[\protect\citeauthoryear{Wu et~al.}{2019}]{Wu19}
\begin{barticle}
\bauthor{\bsnm{Wu}, \binits{Y.W.}},
\bauthor{\bsnm{Reid}, \binits{M.J.}},
\bauthor{\bsnm{Sakai}, \binits{N.}}, \betal:
\batitle{Trigonometric parallaxes of star-forming regions beyond the tangent
point of the Sagittarius spiral arm}.
\bjtitle{Astrophys. J.}
\bvolume{874}(\bissue{1}),
\bfpage{94}
(\byear{2019}).
\doiurl{https://doi.org/10.3847/1538-4357/ab001a}.
\bcomment{\arxivurl{1901.09313} [astro-ph.GA]}
\end{barticle}
\OrigBibText
Wu YW, Reid MJ, Sakai N, et~al (2019) Trigonometric Parallaxes of
Star-forming Regions beyond the Tangent Point of the Sagittarius Spiral
Arm. Astrophysical Journal 874(1):94.
\url{https://doi.org/10.3847/1538-4357/ab001a}, arXiv:1901.09313
[astro-ph.GA]
\endOrigBibText
\bptok{structpyb}
\endbibitem

%b42 ###bbsrt2
%b42 ###
\bibitem[\protect\citeauthoryear{Zhang et~al.}{2005}]{Zhang05}
\begin{barticle}
\bauthor{\bsnm{Zhang}, \binits{Q.}},
\bauthor{\bsnm{Hunter}, \binits{T.R.}},
\bauthor{\bsnm{Brand}, \binits{J.}}, \betal:
\batitle{Search for CO outflows toward a sample of 69 high-mass protostellar
candidates. II. Outflow properties}.
\bjtitle{Astrophys. J.}
\bvolume{625}(\bissue{2}),
\bfpage{864}--\blpage{882}
(\byear{2005}).
\doiurl{https://doi.org/10.1086/429660}
\end{barticle}
\OrigBibText
Zhang Q, Hunter TR, Brand J, et~al (2005) Search for CO Outflows
toward a Sample of 69 High-Mass Protostellar Candidates. II. Outflow Properties.
Astrophysical Journal 625(2):864--882.
\url{https://doi.org/10.1086/429660}
\endOrigBibText
\bptok{structpyb}
\endbibitem



\end{thebibliography}


%%\printdocgrant
\pubnote[print=true]
%%\printRightsRetention

\end{backmatter}
\end{document}

